Compositional Generalization and Decomposition in Neural Program Synthesis

When writing programs, people have the ability to tackle a new complex task by decomposing it into smaller and more familiar subtasks. While it is difficult to measure whether neural program synthesis methods have similar capabilities, what we can measure is whether they compositionally generalize, that is, whether a model that has been trained on the simpler subtasks is subsequently able to solve more complex tasks. In this paper, we focus on measuring the ability of learned program synthesizers to compositionally generalize. We first characterize several different axes along which program synthesis methods would be desired to generalize, e.g., length generalization, or the ability to combine known subroutines in new ways that do not occur in the training data. Based on this characterization, we introduce a benchmark suite of tasks to assess these abilities based on two popular existing datasets, SCAN and RobustFill. Finally, we make first attempts to improve the compositional generalization ability of Transformer models along these axes through novel attention mechanisms that draw inspiration from a human-like decomposition strategy. Empirically, we find our modified Transformer models generally perform better than natural baselines, but the tasks remain challenging.

==> old.tex <==
%%%%
\newpage 

\section{(Old) Introduction}

% Note from Kensen: I like having all the text in one file so Ctrl-F is easier (to make sure terminology is consistent, easier find-replace, etc). But if others prefer splitting up the tex file that's ok too, since we can always move things around later.

When faced with a complex task in nearly any domain, one can use the problem-solving strategy of \emph{decomposition}, i.e., breaking the task into multiple smaller parts, perhaps repeatedly, until each subtask is easy enough to handle. In the artificial intelligence literature, this technique is used in \emph{hierarchical planning} or \emph{hierarchical learning}, where the AI system splits difficult problems into a hierarchy of smaller and smaller tasks.\todo{cite} Closely related is \emph{compositionality}, the notion that ideas, representations, and tasks can be built through compositions of more primitive ones.\todo{cite} For example, in natural language, a finite vocabulary of words with limited individual meanings can be combined to form an infinite number of sentences with different complex meanings. Even the everyday task of ``fry an egg'' is composed of smaller tasks: put a pan on the stove, heat butter or oil in the pan, crack the egg, and so on. For any problem domain that exhibits compositionality, the decomposition strategy is to reverse the composition by identifying the primitive tasks. \ta

Decomposition is especially important within software engineering, where implementations of subtasks can be combined and reused in modular ways. Applying decomposition is a skill so crucial to programming that the first programming course at Stanford University begins teaching decomposition within the first week of class, immediately after introducing basic syntax, the concept of functions, and simple control flow.\todo{cite} 
\charles{Previous sentence: That's a really good example.}
Decomposition can be applied at various levels of the software engineering process, from the high-level design of components and APIs that interface with each other, to the lower-level implementation of functions by calling other helper functions. Well-decomposed code is highly desirable. \charles{It's probably not necessary to go into the succeeding to go into why breaking down a large program into chunks good, maybe we can just give a citation here. Maybe it's enough here to say: good code written by professional developers breaks down a large task into functions, that each solve a subtask. This is clear evidence that} The organization of code into smaller parts reduces cognitive load, making the code easier to read and understand. The smaller units of code allow the programmer to isolate functionality, which aids in debugging and testing. Because most programming languages are compositional, different portions of the code can be composed and reused in different ways, allowing for easier expression of more complex behavior. Finally, decomposition aids in project management and collaboration between programmers, since the subtasks are more straightforward and independent. \charles{The past few sentences are all empirical claims that require evidence, i.e. we should have citations for them or not say them quite so broadly. It's possible that we don't need to give evidence for why this style of writing code makes software engineering better. Maybe the only claim we need to make is "decomposition is a fundamental part of software engineering".}

Despite being a fundamental part of programming, decomposition is not trivial. Often the hardest part of writing code is untangling the requirements and constraints to identify a reasonable decomposition. Best practices for high-level decomposition through the use of design patterns\todo{cite} are still evolving.

Considering the importance of decomposition in programming, it is natural to consider its role in program synthesis, where the goal is to automatically produce code from a specification of what the code should do. It is preferable for a program synthesis system to solve complex tasks by producing code with good decomposition, due to the many benefits provided by decomposition as discussed above.

Search-based program synthesis approaches, especially Programming by Example (PBE) systems, are great at implementing small self-contained tasks such as short Java functions\todo{cite FrAngel}, string manipulation\todo{cite FlashFill and CrossBeam}, and tensor manipulation\todo{cite TF-Coder}. Generally speaking, search-based program synthesizers are designed to compose basic code elements to create more complex programs, and thus they tend to excel at identifying the correct decomposition of the task into basic operations or provided library functions, given enough search budget. However, due to the nature of search within a program space that grows exponentially with respect to the program length, these search-based methods have not had much success generalizing to problems that require more than a few lines of code. The poor \emph{length generalization}
\charles{I am not sure that I am comfortable saying that search-based program synthesis fails to length generalize. TF-Coder fails to generate long programs because it runs out of compute budget. In principle, if you had an exponentially large budget, it would find the correct answer. That's not what is going on when transformers fail to length generalize. Since the two phenomenon have such different causes, I'm not sure that I am fan of describing them by the same technical term.}
ability of search-based program synthesizers suggest that, even though they may solve small compositional tasks, they are not actually using the strategy of decomposition to the fullest---if they were, they could solve much more complex tasks by breaking them into simpler tasks that are easily solved sequentially, where a feasible decomposition is found without the need for an exponential-time search.
\charles{What does it mean for a synthesizer to use decomposition? Just that it does top-down search over programs? I'm not sure that's how we want to define it --- for one, we don't know that top-down search is necessary for synthesis, and for another, there's no mystery about whether a synthesizer is using top-down search or not, we can just look at the code.}

On the other hand, we can similarly question whether neural network-based program synthesizers are actually using decomposition. Some neural program synthesizers, especially those based on large language models,\todo{cite, e.g., Codex} can produce larger amounts of code than search-based synthesizers, but it is unclear how well they can generalize to new \emph{concepts} (e.g., APIs) that are not abundant in the training data. Furthermore, most neural program synthesizers\todo{cite DeepCoder, RobustFill, Codex} are not designed with inductive biases toward a decomposition strategy or toward the compositional nature of code. Finally, neural synthesizers are not yet good at defining multiple functions that work together in a cohesive way to solve a larger problem. In other words, a human programmer still needs to provide expert supervision in the form of decomposing the larger task into subtasks that are simple enough for the neural synthesizer to handle.

How might we measure the decomposition ability of program synthesizers? One approach would be to run the synthesizer on complex tasks with long solutions, and manually judge the synthesizer's output code, looking for a reasonable decomposition. 
\charles{Maybe we don't need the previous sentence? It seems a bit of a straw man.}
Of course, this would be subjective and enormously tedious. Instead, our approach is to identify desirable \emph{compositional generalization properties} that would be present for an approach that uses decomposition. For example, a programming agent (human or not) that uses decomposition would be able to easily generalize to harder tasks requiring the composition of more basic parts, as well as generalize to combining new concepts under learned compositional patterns. \kensen{Maybe add example?} In total, we identified 7 different forms of compositional generalization of varying difficulty, which we can use to quantify decompositional ability along different axes. Good performance on these compositional generalization tasks can be viewed as a strong signal that a program synthesizer is using a decomposition strategy, or at least demonstrates the desired effects of doing so.

We create a suite of benchmark tasks based on two popular datasets, RobustFill\todo{cite} and SCAN\todo{cite}, where each dataset has tasks for each of the 7 forms of compositional generalization we identified. All of the tasks can be used to measure zero-shot and few-shot compositional generalization ability.

We also make first attempts to design neural architectures with decomposition as an inductive bias, where we encourage the model to focus on one subtask at a time. There are a few variations of our approach. Overall, they outperform a baseline Transformer, but no variation is consistently the best at the different generalization tasks. This suggests that the tasks are quite different, and there is much room for improved performance on the benchmark suite.

(Maybe write a bit about how the datasets include multiple parts per problem, with clearly delineated ground-truth ``partial programs'' to aid in training decomposition-aware models. The program specifications are not delineated, so the model needs to learn the decomposition. Suggest that we want to encourage exploration in this research space.)

\section{(Old) Datasets}

Measuring decomposition ability is tricky. We cannot easily interpret the exact steps a neural model takes toward a solution. However, we can measure emergent properties of decompositional thinking. Consider a ``decompositional agent'' (human or not) that writes code using decomposition. Then:
\begin{itemize}
    \item \emph{A decompositional agent is good at length generalization.} After learning how to solve a class of subtasks and how to identify these subtasks within a larger task, the agent should not have great difficulty solving larger and larger compositions of such subtasks. It is natural to use more time or computational power to solve larger compositions, but the effort required should grow roughly linearly with the number of subtasks, and certainly not exponentially.
    \item \emph{When solving a particular subtask, a decompositional agent is (almost) agnostic to the context of other independent subtasks.} After the initial decomposition phase (``hierarchical planning,'' where subtasks must be properly identified or designed to solve the compositional task), each individual subtask can be solved largely independently. Hence, the ability of the decompositional agent to solve an individual subtask should not heavily depend on the other kinds of subtasks or the order that subtasks are solved in. In practice though, it can be good to keep in mind other subtasks for the sake of consistency, learning on-the-fly, and when the other subtasks are used in the solution to this subtask (although it is good practice to not rely on the implementation details of nested subtasks).
    \item \emph{A decompositional agent can generalize the concepts it has learned by applying them in novel ways, as long as those ways are consistent with broader compositional patterns that it has learned.} If the agent knows how to square a number, how to negate a number, and how to negate every number in a list, then it should be able to square every number in a list. It does so by identifying that the task can be decomposed into the form of applying a function (negation or squaring) to every element of a list, and the agent simply needs to swap one concept (negation) for another (squaring).
    \item \emph{Finally, a decompositional agent excels in the few-shot learning setting.} It learns quickly when presented with only a few examples of some novel kind of composition. It is able to identify and generalize patterns in this new kind of composition, without requiring combinatorially many examples of the composition instantiated in different ways.
\end{itemize}

Even if we cannot directly observe a neural model solving complex tasks in a decompositional way, if that model demonstrates excellence in all of the desired ways that we would expect from a decompositional agent, then the model is performing decomposition for all practical purposes. To this end, we have created a benchmark suite of tasks designed to measure these desired properties of a decompositional agent.
